Reflectance study of ice and Mars soil simulant associations -- II. CO$_2$ and H$_2$O ice

We measure the visible and near-infrared reflectance of icy analogues of the Martian surface made of CO$_2$ ice associated in different ways with H$_2$O ice and the regolith simulant JSC Mars-1. Such experimental results obtained with well-controlled samples in the laboratory are precious to interpret quantitatively the imaging and spectral data collected by various Mars orbiters, landers and rovers. Producing and maintaining well-characterized icy samples while acquiring spectro-photometric measurements is however challenging and we discuss some of the difficulties encountered in preparing and measuring our samples. We present the results in the form of photometric and spectral criteria computed from the spectra and plotted as a function of the composition and physical properties of the samples. Consistent with previous studies, we find that when intimately mixed with other materials, including water ice, CO$_2$ ice becomes rapidly undetectable due to its low absorptivity. As low as 5 wt.$\%$ of fine-grained H$_2$O ice is enough to mask entirely the signatures of CO$_2$. Similarly, sublimation experiments performed with ternary mixtures of CO$_2$ ice, H$_2$O ice and JSC Mars-1 show that water, even when present as a minor component (3 wt.$\%$), determines the texture and evolution of the mixtures. We assess the ability of various combinations of spectral parameters to identify samples with H$_2$O, CO$_2$, JSC Mars-1, or various mixtures from their reflectance and orient our study to helping interpret ice and soil reflectance spectra from the Martian surface. From the laboratory spectra, we simulate the colour signal generated by the CaSSIS instrument to allow for direct comparisons with results from this instrument and provide to databases the necessary spectral data to perform the same operations with other instruments.

==> Case_Mars_CO2.tex <==
\section{Martian case study. CRISM observations of the spring sublimation of the northern seasonal polar cap.}
\label{S:Mars}
In 2013, Pommerol et al. \cite{Pommerol:2013} published a survey on the evolution of the appearance of seven northern high-latitude regions during the retreat of the seasonal polar cap. Using data provided by CRISM and HiRISE, they monitored the CO$_2$ and H$_2$O signatures throughout the northern spring of Martian Years (MY) 29 and 30, exploring both spatial and temporal spectral variations. We have selected two of those regions and performed additional spectral and colour analysis on their reflectance spectra. For information related to the acquisition and calibration of the CRISM data, see \cite{Pommerol:2013}.


\subsection{Buzzel (84$^{\circ}$N, 233.2$^{\circ}$E)}
\label{S:6.1}

\begin{figure}[h]
    \centering\includegraphics[width=\textwidth]{Buzzel}
    \caption{Comparison of CRISM measurements of the Martian region of Buzzel to the measurements of the laboratory samples. i) Simplified legend. For the complete legend of the laboratory points see Fig. \ref{Fig:comparison_criteria_legend}. The colours of the Martian points correspond to the dates of measurement as indicated by arrows in the timeline. a) Comparison of the reflectance of the continuum to the H$_2$O index at 1.5 \textmu m. b) Comparison of the reflectance of the continuum and the CO$_2$ index at 1.435 \textmu m. c) H$_2$O index at 1.5 \textmu m compared to the VIS (top) and NIR (bottom) spectral slopes. d) Signal simulated in the RED filter of CaSSIS versus the PAN/RED (top) and BLU/RED (bottom) band ratios. } 
    \label{Fig:Buzzel}
\end{figure}

The first region, referred to as Buzzel, is located at 84$^{\circ}$N and 233.2$^{\circ}$E, beside the north polar layer deposits (NPLD). This region comprises dune fields as well as plain terrains, and has a great density of measurements available from L$_S$ = 7.95$^{\circ}$ to L$_S$ = 88.83$^{\circ}$ in MY29 and from L$_S$ = 52.28$^{\circ}$ to L$_S$ = 82.25$^{\circ}$ in MY30. We have selected a region in-between the dunes to proceed with the same spectral analysis explained in Section \ref{S:Methods}, and finally added the results to the plots shown in Section \ref{R:comparison} for different L$_S$ values (Fig. \ref{Fig:Buzzel}). 

Fig. \ref{Fig:Buzzel}a illustrates the evolution of the reflectance of Buzzel as a function of its water index (at 1.5 $\mu$m). The absolute uncertainty in the reflectance measured by CRISM is about 10$\%$, which has to be taken into account to read the Y-axis of this plot. Right after the spring equinox (L$_S$=0$^{\circ}$), the regions of interest (ROIs) in Buzzel take up the space of the plot with a lack of laboratory points, i.e., around reflectance values of 0.5 and indexes in the range of 0.1-0.5. As spring moves forward, the reflectance and indexes increase, to peak, almost at mid-spring (L$_S$=40$^{\circ}$), at values near 0.6 and 0.5 respectively. App{\'e}r{\'e} et al. proposed two scenarios to explain this water enrichment \cite{Appere:2011}: in the first one, the sublimation of CO$_2$ reveals water-ice grains initially trapped within the CO$_2$, whereas in the second scenario, water condenses progressively on the remaining substrate. From L$_S$=40$^{\circ}$, the signature of water decreases to reach a minimum of $\sim$0.05 almost at the summer solstice (L$_S$=90$^{\circ}$). The decrease in the water signature comes with a drop in the reflectance of about 60$\%$ in the second half of the Spring. During this weakening of the studied parameters, several CRISM measurements fall within the laboratory points that correspond to intimate mixtures of water-ice and JSCM-1, especially during MY30. 

We compare in Fig. \ref{Fig:Buzzel}b the reflectance of the continuum with the absorption signature of CO$_2$ at 1.435 \textmu m. The start of Spring in MY29 (L$_S$=0$^{\circ}$-15$^{\circ}$) marked the strongest CO$_2$ signals; $\sim$25$\%$ stronger than the greatest signals measured in our laboratory samples. We observe a gradual weakening of the sample until L$_S$=39$^{\circ}$, followed by a fluctuation period that lasts until L$_S$=65$^{\circ}$. During that period, the reflectance progressively decreases, however, the carbon dioxide signature goes back and forth. After L$_S$=65$^{\circ}$, the reflectance falls to 0.2 and the signature of CO$_2$ fades away. MY30 shows a similar progression in reflectance, while the decrease in the signature of CO$_2$ seems to be more steady. Hence, at L$_S$=50$^{\circ}$-60$^{\circ}$ the CO$_2$ evaluator remains steady around 0.06, to start fading out from L$_S$=65$^{\circ}$. 
The progressive weakening of CO$_2$ signal does not reflect on the continuum reflectance, which starts fading away when water ice sublimates, as noted in \cite{Pommerol:2013}. The ternary mixtures with SPIPA-B ice reproduce the values observed on Mars, even the increase of carbon signature already discussed in Section \ref{S:Discussion}. 

Figure \ref{Fig:Buzzel}c shows the behaviour of the water index as a function of the spectral slopes. In the near-infrared, most of the points from Buzzel overlap the intimate mixtures of JSCM-1 and water ice (both in MY29 and MY30). The great presence of CO$_2$ ice in the first half of Spring (until L$_S$=40$^{\circ}$) hides the water ice underneath, which is why the corresponding CRISM observations overlap the intimate mixtures with less water fraction. The observations acquired near Summer (L$_S$=$\sim$90$^{\circ}$) fall in the cluster formed by the water frost experiments and the ones containing carbon dioxide but no water ice. In the visible spectral range, the CRISM observations do not follow the trend drawn by the JSCM-1 and water ice intimate mixtures. Instead, the early-spring points (until L$_S$=40$^{\circ}$) lie around the frozen soils, and intimate mixtures laboratory points and redden after L$_S$=40$^{\circ}$. None of our laboratory samples shows such red values (60-70$\%$/100 nm) for water indexes of about 0.5, or, in other words, such a great water signature for VIS slopes between 60-70$\%$/100 nm. Hypothetically, intimate mixtures of JSCM-1 and water ice grains bigger than SPIPA-B could match the observations from the Martian surface, but in that case, the water indexes would get too deep compared to the observed ones (Fig. \ref{Fig:Buzzel}a). Close to the summer solstice (L$_S$=90$^{\circ}$), the CRISM observations overlap our JSCM-1 samples with water frost. The CRISM observation at MY29 (L$_S$=88$^{\circ}$) and the one at MY30 (L$_S$=82$^{\circ}$) show slightly different slopes for the same index (and, from Fig. \ref{Fig:Buzzel}, equal reflectance). Slight variations in condensed water frost, as well as the presence of finer or coarser dust grains,  could explain this behaviour. 

We now analyse how the colours of Buzzel would look like measured with CaSSIS (Fig. \ref{Fig:Buzzel}e). Looking at both the PAN/RED and BLU/RED ratios, we distinguish two clusters; the first one contains every point from the spring equinox (L$_S$ = 0$^{\circ}$) to around L$_S$ = 70$^{\circ}$ and shows reflectance values in the RED between 0.4 and 0.5. The points closest to Summer forms the second one (L$_S$ = $\sim$90$^{\circ}$), whose reflectance in the RED filter is roughly 0.2. Compared to the laboratory samples, these summer observations are about 20$\%$ and 35$\%$ brighter in the PAN and BLU filter respectively. The other group of observations fall in the vicinity of our frost experiments in the PAN/RED plot, whereas they do not overlap our samples in the BLU/RED plot, since they appear $\sim$40$\%$ redder than our frost experiments. 

From the plots in Fig. \ref{Fig:Buzzel} we see that for Buzzel:
\begin{itemize}
\item If condensation of frost (understood as fresh, light ice) caused the maximum spectral enrichment of water observed at L$_S$=39.12$^{\circ}$, we would expect a greater increase in the reflectance of the continuum (Fig. \ref{Fig:Buzzel}a). Besides, we would also expect a greater slope-flattening-to-index-increasing in Fig. \ref{Fig:Buzzel}c (VIS), and a deviation from the trend determined by the previous measurements in the Fig. \ref{Fig:Buzzel}c (NIR). The fact that none of these terms is satisfied points to a scenario where the maximum enrichment of water is due to the progressive revelation of water ice trapped in the CO$_2$ instead of to frost condensation.

\item Compared in the visible range, the CRISM observations acquired after L$_S$=80$^{\circ}$ differ slightly in MY29 and MY30. Hence, we detect water frost-like signal (i.e., almost no effect on the NIR range and marked impact in the VIS colours) in the observation of MY30 (L$_S$=$\sim$82$^{\circ}$) compared to the one in MY29 (L$_S$=$\sim$88$^{\circ}$). This difference is weaker than the one observed between our dry powders and the first step of frost deposition, which was estimated to a micrometre layer. The possibility that in the last observation of MY30 there was some water frost left cannot be ruled out, in which case the regolith in Buzzel would have a slightly blue NIR slope. 
\end{itemize}


\subsection{Kolhar (85$^{\circ}$N 0$^{\circ}$E)}
\label{S:6.2}

\begin{figure}[h]
    \centering\includegraphics[width=\textwidth]{Kolhar}
    \caption{Comparison of CRISM measurements of the Martian region of Kolhar to the measurements of the laboratory samples. i) Simplified legend. For the complete legend of the laboratory points see Fig. \ref{Fig:comparison_criteria_legend}. The colours of the Martian points correspond to the dates of measurement as indicated by arrows in the timeline. a) Comparison of the reflectance of the continuum to the water index at 1.5 \textmu m. b) Comparison of the reflectance of the continuum and the of CO$_2$ index at 1.435 \textmu m. c) Water index at 1.5 \textmu m compared to the VIS (top) and NIR (bottom) spectral slopes. d) Signal simulated in the RED filter of CaSSIS versus the PAN/RED (top) and BLU/RED (bottom) band ratios.} 
    \label{Fig:Kolhar}
\end{figure}

The second region, located at 85$^{\circ}$N 0$^{\circ}$E, is a dune field that has received the informal name of Kolhar. Kolhar is of particular interest because it is the region located at highest latitude from the ones studied in \cite{Pommerol:2013}. Also, it displays a decrease of the water-ice signature between L$_S$ = 23.42$^{\circ}$ and L$_S$ = 40.80$^{\circ}$ (MY29) that has been associated to either the apparition of fine frost on the surface or the formation of clouds in the atmosphere \cite{Pommerol:2011}. To see whether our analysis can shed light on this question, we have delimited two ROIs in Kolhar: one in a dune itself and another one in the substrate adjacent to it, between two dunes. The results are shown in Fig. \ref{Fig:Kolhar}.

In Fig. \ref{Fig:Kolhar}a, we observe a similar evolution of the surface as the one seen in Buzzel regarding the reflectance of the continuum and water signature. The main difference is that, while in Buzzel the maximal water signature was measured around L$_S$ = 40$^{\circ}$, in Kolhar, L$_S$ = 40$^{\circ}$ marks a local minimum of the water signal, and the maximum signal is measured at L$_S$ = $\sim$65$^{\circ}$ in MY29 and L$_S$ =$\sim$60$^{\circ}$ in MY30. In MY 29, the substrate presents greater water signature and reflectance than the dune (except in L$_S$ = 40$^{\circ}$), which may be indicative of the presence of more water ice mixed within the regolith. Both in MY29 and MY30, the substrate appear brighter for similar index around the summer solstice (L$_S$ = 90$^{\circ}$), which could be attributed to the presence of water frost or a difference ---mineralogical or in size fraction--- of the two surfaces. 

We follow the evolution of the CO$_2$ spring signature in Figure \ref{Fig:Kolhar}b. Some of the points are missing, since the formula employed resulted in the non-detection of CO$_2$ signatures. At same L$_S$, the surface shows CO$_2$ indexes greater than 0.2 and reflectance values lower than 0.4 in the first half of the Spring (until L$_S$ = 45$^{\circ}$), and indexes smaller than 0.05 with reflectance values lower than 0.4 the second half of the Spring. L$_S$ = $\sim$45$^{\circ}$ also means a change in the relative amount of CO$_2$ ice between the dunes and the substrate: the latter presents a signal of CO$_2$ $\sim$20$\%$ stronger than the dune. As Spring moves forward, the difference between regions diminishes, and from L$_S$ = 45$^{\circ}$ until the end of Spring, the CO$_2$ signature of the dune is stronger than the one of the substrate. 

The evolution of the water index compared with the VIS and NIR spectral slopes reproduces the patterns observed in the region of Buzzel (\ref{Fig:Kolhar}c). Hence, while the CRISM data align with our intimate mixtures of JSCM-1 and water ice in the NIR range, we do not observe such a clear alignment in the visible VIS range. Furthermore, Fig. \ref{Fig:Kolhar}c provides new information, non-inferable from Fig. \ref{Fig:Kolhar}a: first, the point at L$_S$ = 40$^{\circ}$ (MY 29) shows a reddening of the surface both in the VIS and in the NIR, which suggests that dust (either on the surface or in a cloud) could be the reason of the decrease in the water signal observed in Fig. \ref{Fig:Kolhar}a. Second, the point at L$_S$ = 47$^{\circ}$ (MY 30), which does not stand out in Figure \ref{Fig:Kolhar}a, distinguishes itself from the other points by showing a VIS spectral slope 30$\%$ redder than the following observation. None of these points deviates from the trend followed by the other measurements in the NIR. Third, the substrate appears $\sim$30$\%$ redder than the dunes, which indicates that the higher reflectance observed in Fig. \ref{Fig:Kolhar}a is not due to water frost.

Finally, Fig. \ref{Fig:Kolhar}d shows these observations as would have been seen with CaSSIS. In the PAN/RED plot, the CRISM observations move from the points of water frozen soils and JSCM-1 and CO$_2$ measurements towards the ones of water frost and water ice and JSCM-1 experiments. Again, the substrate and the dune show different colours close to the summer solstice (L$_S$ = 90$^{\circ}$), with the substrate being redder than the dune. The surface of Kolhar shows a more significant change in the BLU/RED ratio than the surface of Buzzel. In MY29, the first measurements (L$_S$ = $\sim$20$^{\circ}$) indicate a bluing of the surface as water is revealed, followed by a substantial reddening at L$_S$ = 40$^{\circ}$, as repeatedly observed. From L$_S$ = 50$^{\circ}$, the brightness of the surface decreases faster in the RED than in the BLU filter, which corresponds to the increase of the water signal observed in Figure \ref{Fig:Kolhar}a. From L$_S$ = $\sim$80$^{\circ}$, the situation reverts itself, and the RED reflectance dominates. Around Summer (L$_S$ = 90$^{\circ}$), the observations of the dune show bluer colours than the ones of the substrate. Besides, Figure \ref{Fig:Kolhar}d confirms the contrary behaviour of the points around L$_S$ = 40$^{\circ}$ to the one of water frost; in short wavelengths, they are redder than the previous and following measurements. 

From the plots in Fig. \ref{Fig:Kolhar} we see enough pieces of evidence to conclude that the decline of the water signal at around L$_S$ = 40$^{\circ}$ was not due to the condensation of frost: \textit{i)} the amount of frost needed to decrease the water index by 30$\%$ is expected to boost the reflectance of the continuum more than the 10$\%$ observed in the CRISM data, \textit{ii)} the observation at L$_S$ = 40$^{\circ}$ is redder than the majority of the other observations, and \textit{iii)} the amount of frost needed to reduce the water index by 30$\%$ should be enough to deviate the points from the trend observed in the near-infrared part of Fig. \ref{Fig:Kolhar}c. Therefore, the hypothesis of frost can be here ruled out to favour the one that proposes the presence of clouds of aerosols in the atmosphere. 

Furthermore, we have seen that around the summer solstice (L$_S$ = 90$^{\circ}$), substrate and dune show terrains of different properties. Hence, the surface of the substrate is brighter and redder than the one of the dune. The finest fraction of JSCM-1 has been shown to be redder and brighter than its bigger counterpart \cite{Yoldi:2018a}. Since wind transports easily fine grains, there could be a coating of fine dust on the substrate, which would cause the measured variations. Such differences in grain size would imply distinct thermal properties of the soil (e.g. lower thermal inertia of the fine grains), which could also be behind the disruption of H$_2$O ice, only observed on the dunes \cite{Pommerol:2013}. 


\subsection{Discussion and perspectives}
\label{S:6.3}
Some of the discrepancies between our laboratory samples and the Martian observations can be explained in the frame of Kieffer's model, which states that in early spring, CO$_2$ ice is present in the form of meter-sized and translucent slabs \cite{Kieffer:2006}. At the North pole of Mars, the dune fields are also covered with a translucent slab of CO$_2$ \cite{Kieffer:2001}. Recent laboratory measurements have shown that, under Martian conditions of temperature and pressure, CO$_2$ tends to condense as a transparent slab \cite{Anya:2018}. Such a thick slab of carbon dioxide would explain the CO$_2$ indexes measured with CRISM compared to our laboratory samples (Figs. \ref{Fig:Buzzel}b and \ref{Fig:Kolhar}b). %Furthermore, the presence of a slab of ice together with the low incidence light of the beginning of Spring could result in a rise of reflectance caused by the forward scattering, which could explain the relatively high reflectance from Buzzel and Kolhar compared to laboratory samples of same water signature. 

Comparisons between the visible and near-infrared slopes (Figs. \ref{Fig:Buzzel}c and \ref{Fig:Kolhar}c) or between the BLU, PAN and RED filters (Figs. \ref{Fig:Buzzel}d and \ref{Fig:Kolhar}d) evince that our laboratory samples resemble more the Martian soils in the NIR than in the VIS range. An explanation could be that, as discussed in Section \ref{S:Discussion}, we are more sensitive to the texture at less absorptive wavelengths and the composition in more absorptive wavelengths (NIR). This could explain why, in the comparison of the water index with the spectral slopes, the CRISM observations of Buzzel overlap the laboratory intimate mixtures in the NIR range, but plot around the frozen soils in the VIS range. 

Nevertheless, some of the differences between the Martian soils and the laboratory samples cannot be explained only by the different sensitivities of the spectral ranges to the texture. In particular, during most of the spring, Buzzel and Kolhar show a RED reflectance as high as our intimate mixtures with 75wt$\%$ of ice, but show a BLU reflectance as low as the intimate mixtures with 10wt$\%$ of ice. At the end of the spring, however, the CRISM observations fall in the RED-to-BLU/RED ratios of our samples, indicating that the discrepancy between the CRISM observations and our samples is not due to a wrong choice of soil simulant. The presence of aerosols in the atmosphere could also contribute to a more significant reddening at short than at long wavelengths, but further research is needed to understand this. 

With the first ternary mixtures that we have produced, we can simulate the weakening of the CO$_2$ signature observed at the Martian surface around the North pole. In particular, we best overlap the CRISM observations with the SPIPA-B samples in the second half of the season (i.e., from L$_S$ = 45$^{\circ}$), once the deposits of water ice and dust are thick enough to start masking to weaken the CO$_2$ signature. We also reproduce the strengthening of the water signature and the start of the weakening, although we would have needed more time to attain values as weak as the ones measured with CRISM. The addition of insulation cycles could help reproducing the steeper decrease of the water index and the transient increase of reflectance, respectively.

Our ternary mixtures do not reproduce, however, the initial increase of reflectance observed with CRISM. This can be explained by the fact that our ternary mixtures were composed of CO$_2$ snow, showing a great albedo, while the CO$_2$ ice on these regions is expected to be present as a slab, as mentioned before. Thus, the brightest component of our ternary samples is the CO$_2$ snow, while the brightest one on Mars would be the water frost. 

\begin{figure}[h]
    \centering\includegraphics[width=\textwidth]{Buzzel_composite}
    \caption{RGB colour composite: the continuum reflectance has been used in the red channel, the CO$_2$ index in the green channel and the H$_2$O index in the blue channel. a) CO$_2$/H$_2$O/JSCM-1 in t$_6$. Stretch: R(0.2-0.95), G(0.025-0.125), B(0.3-0.8). b) Buzzel in MY30, L$_S$ = 60.7$^{\circ}$. Stretch: R(0.318-0.520), G(0.214-0.306), B(0.339-0.575). This image has been reproduced from \cite{Pommerol:2013} under the licence number 4333701425893.}
    \label{Fig:Buzzel_composite}
\end{figure}

Figure \ref{Fig:Buzzel_composite} compares composite images of our ternary mixtures (in t$_{6}$) and of Buzzel in MY30, L$_S$ = 60.7$^{\circ}$. In these images, the R, G and B channels are filled with the continuum reflectance, CO$_2$ and H$_2$O indexes respectively. Since the stretch values are different (see caption of Fig. \ref{Fig:Buzzel_composite}), the direct comparison between colours is not possible. However, we can see some similarities between the images, for instance, how CO$_2$ remains in the creases of our samples, in the same way it follows the topography in Buzzel. The sample of SPIPA-A is covered by water, as is the top of the north polar layer, visible at the bottom-right of Buzzel.

Finally, as we have discussed in Section \ref{S:Discussion}, Singh and colleagues modelled the spectra of various sizes of CO$_2$, obtaining a red slope at wavelengths shorter than 0.5 \textmu m, which is steeper for big particle sizes \cite{Singh:2016}. Even if we do not measure such red slopes, we start observing, only for slabs, a slightly higher reflectance in the RED than in the BLU filter of CaSSIS. If laboratory measurements confirm this difference, this could be a property to explore, since it could be used to discriminate CO$_2$ from H$_2$O in the visible range. 



